Tuple-oriented Compression for Large-scale Mini-batch Stochastic Gradient Descent

Data compression is a popular technique for improving the efficiency of data processing workloads such as SQL queries and more recently, machine learning (ML) with classical batch gradient methods. But the efficacy of such ideas for mini-batch stochastic gradient descent (MGD), arguably the workhorse algorithm of modern ML, is an open question. MGD's unique data access pattern renders prior art, including those designed for batch gradient methods, less effective. We fill this crucial research gap by proposing a new lossless compression scheme we call tuple-oriented compression (TOC) that is inspired by an unlikely source, the string/text compression scheme Lempel-Ziv-Welch, but tailored to MGD in a way that preserves tuple boundaries within mini-batches. We then present a suite of novel compressed matrix operation execution techniques tailored to the TOC compression scheme that operate directly over the compressed data representation and avoid decompression overheads. An extensive empirical evaluation with real-world datasets shows that TOC consistently achieves substantial compression ratios by up to 51x and reduces runtimes for MGD workloads by up to 10.2x in popular ML systems.

==> Makefile <==
### Makefile --- 

TARGETS = paper

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> discuss.tex <==
\section{Discussion}
{\bf Redundancy in data}: 
Some datasets e.g. [] have little redundancy inside and cannot be efficiently compressed using TOC compression. Nevertheless, we have tested other compression methods for example [] and found that dataset like [] cannot be compressed efficiently using these compression methods either. In this case, using the uncompressed data as the input seems to be the reasonable way to do SGD.\par

{\bf BGD vs. SGD}:
Although TOC compression is proposed aiming at performance optimization during SGD in machine learning, it is also suitable for BGD. In fact, the performance improvement is more significant in the BGD case because there is more redundancy if the training dataset is not sliced into mini-batches.\par

{\bf Multi-layer Neural Network}:
In our experiment sec X, we use a neural network with only one hidden layer. Given the proliferation of deep learning, it is worthwhile to consider how to apply TOC compression in deep neural network, which has many hidden layers.  Although TOC compression and its corresponding matrix operation accelerations can only be applied to the first hidden layer in this case, it is still beneficial to apply TOC because it significantly reduces the memory footprint required by the data and the I/O time needed. How to optimize the computations in the middle layers can be an interesting future work. In addition, our technique can be applied to other variants of neural network, for example convolutional neural network, recurrent neural network, etc.\par



==> overview.tex <==
We now discuss how we use coding techniques to accelerate ML algorithms. We use the classical 
Lloyd algorithm for k-means clustering as a detailed running example and then generalize our ideas.

% In Section~\ref{sec:overview:paradigm}, we present a paradigm for accelerating machine learning methods using coding.
% In Section~\ref{sec:overview:lloyd} we use the Lloyd algorithm to illustrate opportunities in using
% source coding for acceleration. We then generalize these ideas in Section~\ref{sec:overview:generalizations}
% so that it applies to other machine learning problems. We close this section with a discussion
% in Section~\ref{sec:overview:discussions} of the opportunities associated with applying our ideas
% to deep learning with neural nets, which is an interesting ongoing work. %though we have not been able to extend our ideas to handle them.

\subsection{A Paradigm for Accelerating Machine Learning using Coding}
\label{sec:overview:paradigm}
\begin{figure}[!htb]
\centering
\includegraphics[width=0.6\columnwidth]{plots/overview_plot.pdf}
\captionof{figure} {An illustration of our paradigm for using coding to accelerate ML algorithms.}
\label{fig:overview}
\end{figure}

We first explain our paradigm for accelerating ML algorithms using coding.
Common with such accelerations for low-level data processing, our goal is to \textit{encode} the input data
and then modify the computations to operate directly over the {\em encoded data}.
Typically, for ML algorithms, the structure of computations is more complicated
than that of the low-level data processing operations. For most ML techniques,
we have a loss function that is determined by the model structure
(for example, the logistic loss for logistic regression), the model parameters,
and the input data points. These pieces jointly determine the values of the loss function
for date points in the training set. Then, an optimizer updates the model (typically, iteratively)
based on the loss until a convergence criterion is met.
In the end, the final model parameters are output.

Figure~\ref{fig:overview} illustrates our paradigm: the codewords, instead of the raw data input, 
are used as inputs to an ML algorithm along with its model parameters and model structure.
Then, an optimization algorithm iteratively optimizes the model.
From this paradigm, we can see that a key challenge is that the effectiveness of the encoding in 
improving runtime performance depends on {\em both the model structure (most importantly, how 
the loss function is defined)} and {\em how the optimization algorithm updates the model during 
the evaluation steps of the loss function}.

\subsection{Running Example: Lloyd's Algorithm}
\label{sec:overview:lloyd}

We use the basic version of Lloyd's algorithm for k-means to illustrate our ideas.
Given a training set $S$ of $m$ data points in a $d$-dimensional space, this algorithm obtains $k$ 
clusters under the $L_2$-distance metric. Note that Lloyd's algorithm is iterative. There are 
three main computations in each iteration. First, given a set of clusters $C_1, C_2,\cdots, C_k$ 
and their corresponding centroids $w_1, \dots, w_k$, we compute the \textit{loss function}
for each $x$ and each $w_i$:
\begin{align}
  \label{eq:k-means-loss}
  \ell(w_i, x) = \|w_i - x\|_2^2 = \sum_{l=1}^d(w_{i,l} - x_l)^2,
\end{align}
Here, $w_{i,l}$ is the $l$-th component of centroid $w_i$, and $x_l$ is the $l$-th component (feature) of $x$. 
Second, each data point is assigned to the cluster $C_j: j \in \arg\min_{i} \ell(w_i, x), i = 1, \dots, k$. 
This is known as the {\em assignment step} for $x$; we assign each $x$ to its ``best current'' cluster. 
Finally, $w_i$ is \textit{updated} as $w_i = \sum_{x \in C_i}{x} / |C_i| $.   
Overall, $O(mkd)$ arithmetic operations are performed per iteration.

%TODO: AK: What is the point of this row-column discussion? It looks like a needless distraction.
\eat{
Our first observation is that, while the above description of the assignment step
describes computations in a row-wise access pattern 
(i.e. we evaluate $\ell(w_i, x)$ for a {\em fixed} $x$ and over all $w_i$), we can also view this computation
from a column-wise, perspective, and equivalently view the computation as {\em fixing a single $w$ in $\{w_1, \dots, w_k\}$,
  and computing $\ell(w, x_j)$ for every $x_j$ ($j=1, \dots, m$) in $S$.}
}

\noindent\textbf{Opportunity I: Exploiting ``Data Redundancy'' in the Training Data}.
We now arrive at our first key observation:
\textit{in many datasets, there are often a lot of ``data redundancies'' among the tuples}. 
In other words, the feature vectors of two examples, $x_i$ and $x_j$ may share values.
Since the computation of $\|w - x_j\|^2$ can be {\em decomposed} into computations over individual 
components (Equation (\ref{eq:k-means-loss})), this implies that we can effectively leverage 
such data redundancy among the tuples in the training set to avoid {\em redundant computations}.
More specifically, given a coding scheme with encoding function $enc$ and decoding 
function $dec$, we define the {\em encoded loss function} as follows:

\begin{definition}[Encoded Loss Function]
  Given a coding scheme, the encoded loss function $\widehat{\ell}$,
  which receives two parameters, a hypothesis $w$ and a codeword $enc(x)$ of $x$, is defined as
  $\widehat{\ell}(w, enc(x)) = \ell(w, x)$.
\end{definition}

Now, suppose that we use a coding scheme to encode the training set $S$ and that all data 
points can be encoded using only a small universe of $t$ words, $U = \{c_1, \dots, c_t\}$, 
where $t \ll m$. In other words, for every $j$, $enc(x_j)$ can be represented as a tuple 
$\langle c^j_{i_1}, c^j_{i_2}, \dots, c^j_{i_{s}} \rangle$:
for some $i_1, \dots, i_s \in \{1, \dots, t\}$.
Then, {\em $\widehat{\ell}(w, enc(x))$ can be computed without decoding.}
By remembering the squared $L_2$-distance between $c^j_{i}$ and the 
corresponding component of $w$ in a {\em cache table} $T$,
we can compute $\widehat{\ell}(w, enc(x))$, which is $\ell(w, x)$,
using $s$ queries to $T$. Note that $T$ is of size $kt$
where we remember for every $w_i$ and every $c_s$,
the squared $L_2$-distance between $c_s$ and the corresponding parts in $w$.
Filling $T$ takes at most $O(tkd)$ arithmetic operations.
Note that $tkd \ll mkd$ as $t \ll m$.

Since the {\em average} number of words $d'$ to encode $x_j$ is much smaller than $d$
(i.e. $d' \ll d$), we can compute {\em all} $\ell(w_i, x_j)$,
using $\widehat{\ell}(w_i, enc(x_j))$ and $T$,
with a total of at most $O(tkd + mkd')$ arithmetic operations.
This is potentially much smaller than $O(mkd)$ as $t \ll m$ and $d' \ll d$.

\noindent\textbf{Opportunity II: Exploiting ``Redundancies'' in the Codeword Universe}.
Until now, our discussion applies to {\em any} source coding scheme. However, we note that
for the special class of {\em prefix source coding}, such as LZW,
we can exploit an additional opportunity. Specifically, for prefix codes,
the universe $U = \{c_1, \dots, c_t\}$  has the essential property that for $c, c' \in U$,
{\em $c$ can be a prefix of $c'$}.
Furthermore, this prefix relationship is encoded in the prefix tree
where each tree node corresponds to a word $c \in U$, and there is a tree edge from $c$ to $c'$
if $c$ is a prefix of $c'$. This observation leads to the second opportunity for acceleration:
{\em We can fill in the cache table $T$ faster than filling them separately.}
Specifically, once we compute the distance between $c$ and $w$,
we can {\em reuse} the result to compute the distance between $c'$ and $w$,
instead of redoing the arithmetic operations on the prefix $c$.
As a result, one can fill the table $T$ by {\em following the topological order,
 that is level by level, of the prefix tree}, exploiting the prefix redundancy.
As a result, one can aim to fill in $T$ with a total number of $N  \ll O(tkd)$ arithmetic operations.
This gives the final arithmetic complexity $O(N + mkd')$, combining both opportunities,
which satisfies that $N + mkd' \ll tkd + mkd' \ll mkd$.

\subsection{Generalizations}
\label{sec:overview:generalizations}
We now extend the ideas from the last subsection to GLMs.

\noindent\textbf{Unification.} We begin by unifying the above two opportunities for the Lloyd's algorithm.
We have two observations: (1) In both cases, the {\em core task} is to evaluate a certain function $f$
over a dataset $D = \{z_1, \dots, z_n\}$. In the first case, $D$ is the training set $S$,
and in the second case $D$ is the universe of the coding scheme $U$.
(2) Suppose that the coding scheme has encoding function $enc$ and decoding function $dec$.
Observe that what is common to both opportunities is that $f$ is ``decomposable'' in the sense that
for any $z \in D$, if $z = z_1 \circ z_2$ (where $\circ$ is the concatenation operator),
then $f(z) = F(f(z_1), f(z_2))$ where $F$ is some combining function.
In the Lloyd's algorithm, for both opportunities, $f$ is the squared $L_2$-distance function $f(\cdot) = \ell(w, \cdot)$
(strictly speaking, one should understand this as follows:
if $enc(x)=\langle c_1,\dots,c_s \rangle$, then $\ell(w, c_1)$ is defined as
the squared 2-norm distance between $dec(c_1)$ and {\em corresponding components} in $w$).
Note that we can replace the $L_2$-distance function by any other common distance function,
such as the $L_p$-distance, and the same argument goes through.

Now, with both (1) and (2), if there is significant data redundancy in $D$,
we can hope to accelerate $f$ on $D$ using our cache table.
In the first opportunity for Lloyd's algorithm, there is redundancy because $D$ is the entire training set.
In the second opportunity, $D$ is $U$ and there is redundancy in $U$ as exposed by the prefix tree.

\noindent\textbf{Generalization to GLMs.}
We note that common optimization algorithms for training GLMs are based on gradient methods,
for example {\em steepest descent}, {\em conjugate gradient descent}, or {\em L-BFGS}.
For these optimization algorithms, we are in a similar situation as the Lloyd's algorithm
by just replacing the {\em $L_2$-distance} function by the {\em inner product} function.
As a result, the same two opportunities can be exploited for GLMs with these algorithms as well.

\subsection{Discussion}
\label{sec:overview:discussions}
We have shown how to exploit the same opportunities to use coding techniques to accelerate 
both k-means trained with the Lloyd's algorithm and GLMs trained with gradient methods. This is intriguing, 
and somewhat surprising, because k-means and GLMs are superficially quite different ML techniques.
We are encouraged by this result, as to the best of our knowledge, this is the first case to expose the 
opportunities in accelerating multiple ML algorithms using the same coding techniques. Not only do we
find that such acceleration is {\em possible}, but that there are also {\em common structures} that can be 
exploited in two fundamental and different ML algorithms.

It is natural then to wonder if our ideas can be extended to more complicated model structures and
other optimization algorithms. For example, one could consider kernel methods
with appropriate convex optimization algorithms.
Even more ambitiously, one could consider deep convolutional neural networks trained
with stochastic gradient descent. We are currently exploring these ideas and
while we do not have answers to these other models yet, we suspect there could be similar
\textit{structures} in those models too that can be exploited using coding techniques.
For example, in a convolutional neural network, this might be possible
as the same small kernel is used in all sliding windows in one  convolutional layer
and the input data also has high redundancy~\cite{nielsen15, Goodfellow-et-al-2016, NIPS2012_4824}. 
Overall, we hope our initial ideas and results presented in this paper spur more interest in the community to 
systematically explore such techniques.

\noindent\textbf{Comparisons with Data Sketching}.
Our discussion so far may remind astute readers about data sketching techniques such as
Gaussian Random Projection~\cite{bingham2001random}, where we ``compress'' the data into lower dimensions,
and thus save computation and storage costs. To this end, we have the following points:
{\bf (1)} Data sketching techniques are ``data independent''
(e.g. we apply a random linear transformation $A$ to the data vectors,
where $A$ is sampled independently of the data), while our technique is ``data dependent.''
{\bf (2)} Our technique guarantees that
``exactly the same thing is learned as without our technique.'' Data sketching techniques,
on the other hand, guarantees ``approximate'' utility with respect to a specific measure,
such as distances between points or test accuracy.
In that sense, our guarantees of losslessness are stronger.
{\bf (3)} Intriguingly, some data sketching techniques can also be applied together with our technique.
For example, with a linear transformation $A$, one may hope that $Ax$ and $Ax'$ have similar redundancies
if $x$ and $x'$ have a lot of redundancies.
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> tc-learning.tex <==
We now explain how we execute Lloyd/GLM directly on our coded data representation. Since we avoid explicit decoding costs, we call our approach TOC-Based Learning (TOC-Learning for short).

\eat{
The first subsection introduces the basic version of TOC-Learning to give the picture of our solution. The second subsection discusses an efficient way to \textbf{precompute} pair-wise distances/inner-products between dictionary entries and centroids/weight for k-means/GLMs. The last subsection discusses how to efficiently \textbf{update} dictionary entries into the centroids/weight for k-means/GLMs.
}

\subsection{Basic TOC-Learning}
\vspace{1mm}
\noindent \textbf{TOC-Lloyd.}
One iteration of TOC-Lloyd is presented in Algorithm~\ref{alg:kmeans-decoding}. At each iteration, we pre-compute the pair-wise squared distances between the dictionary entries and centroids and store them in the 2-dimensional array \textbf{B}. Note that the starting index for each dictionary entry is used to align the features of the dictionary entry with the correct feature dimensions in the centroids. The notation $c_{|e.values}$ means that only the dimensions corresponding to the features present in $e.values$ are used. The partial distances are then used while computing the full distances between the data points and centroids. The array $\textbf{DC}$ tracks how many times each dictionary entry needs to be added (equivalent to adding the examples directly) when computing the new centroids. Thus, TOC-Lloyd might avoid a lot of computational redundancies in both the distance computations and centroid updates.


\vspace{1mm}
\noindent \textbf{TOC-GLM.}
One iteration of TOC-GLM with gradient descent is presented in Algorithm~\ref{alg:Compress_LogisticRegression}. At each iteration, we pre-compute the partial inner products between the dictionary entries and the weights and store them in array \textbf{B}. Again, the notation $w_{|e.values}$ means only the dimensions corresponding to the features present in $e.values$ are used. Then, the gradient is computed in one pass over the compressed data, reusing the pre-computed inner-products. We also aggregate the scalar values after applying the scalar function $g$ for each dictionary entry and update the weights by using each dictionary entry once. Recall that $g(a,b)$ is GLM-specific, e.g., for logistic regression it is $-b/(1+exp(ab))$, while for linear regression, it is $(a-b)$. Overall, TOC-GLM might avoid a lot of computational redundancy in the inner product computations and weight updates.

\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \Input{Compressed \textbf{T'}, Dict.~\textbf{D}, Centroids \textbf{C}}
    //Initialize new centroids \textbf{C'}, \textbf{B}, \textbf{DC} \\
    \For {each $e$ in \textbf{D}} { 
        \For {each $c$ in \textbf{C}} {
            $\textbf{B}[e.code, c.CID] = l_2(e.values - c_{|e.values})^2$ \\
        }
    }
    \For {each $t$ in \textbf{T'}} {
        \For {each $c$ in \textbf{C}} {
            $s_c$ = 0 \\
            \For {each $e$ in $t$} {
                $s_c$ += $\textbf{B}[e.code, c.CID]$
            }
        }
        $\hat{c}$ = $\textnormal{argmin}_{c \in \textbf{C}} s_c$\\
        $Count[\hat{c}.CID] += 1$\\
        \For {each $e$ in $t$} {
            $\textbf{DC}[e.code, \hat{c}.CID]$ += 1
        }
    }
    \For {each $e$ in \textbf{D}} { 
        \For {each $c$ in \textbf{C'}} {
            $c_{|e.values}$ += $e.values \times \textbf{DC}[e.code, c.CID]$
        }
    }
    \For {each $c$ in \textbf{C'}} { 
        $c.x = c.x / Count[c.CID]$
    }
\caption{One Iteration of TOC-Lloyd}
\label{alg:kmeans-decoding}
\end{algorithm}


\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \Input{Compressed \textbf{T'}, Dict. \textbf{D}, Weights $w$, Labels $Y$}
    //Initialize new gradient $G$, \textbf{B}, \textbf{DW} \\
    \For {each $e$ in \textbf{D}} {
        $\textbf{B}[e.code] = w_{|e.values}' e.values $ \\
    }
    \For {each $t$ in \textbf{T'} \textnormal{and corresponding} $y$ in \textbf{Y} } {
        $z = 0$\\
        \For {each $e$ in $t$} {
            $z$ += $\textbf{B}[e.code]$
        }
    
        $z = g(z, y)$ \hfill //GLM-specific gradient function $g$\\
        \For {each $e$ in $t$} {
            $\textbf{DW}[e.code]$ += $z$
        }
    }
    \For {each $e$ in \textbf{D}} {
    $G_{|e.values}$ += $e.values \times \textbf{DW}[e.code]$
    }
\caption{One Iteration of TOC-GLM}
\label{alg:Compress_LogisticRegression}
\end{algorithm}


\subsection{Exploiting Redundancies in Codewords Universe}
\noindent \textbf{Efficient Precomputing}.
We now explain how we efficiently precompute the distances/inner-products between dictionary entries and centroids/weights. 
These precomputations happen in lines 2-4 in Algorithm~\ref{alg:kmeans-decoding} and lines 2-3 in Algorithm~\ref{alg:Compress_LogisticRegression}.
There are two structures that we leverage to achieve this: the prefix tree structure of the dictionary in TOC, and the structure of the function we evaluate on the dictionary entries.

\noindent \textbf{Structure I:}
TOC stores the dictionary entries in a prefix tree. That is, a dictionary entry $(start\_idx, [x_0, x_1, ..., x_n])$ will be stored as a path of nodes starting from root. Note that $start\_idx$ will also be stored as a tree node (with special indicating tag).

\noindent \textbf{Structure II:} The functions $dist$/$weighted\_sum$ over dictionary entries for Lloyd/GLM respectively are decomposable. Let $X$ be a dictionary entry, $X'$ be its longest prefix, and $c$ be the last attribute,
\begin{equation*} \label{eq:prefix-reuse}
    dist(X) = dist(X') + dist(c)
\end{equation*}
\vspace{-4mm}
\begin{equation*}
    weighted\_sum(X) = weighted\_sum(X') + weighted\_sum(c)
\end{equation*}

Thus, we evaluate the dictionary entries in the topological/breadth-first traversal order of the prefix tree. Each time we evaluate a tree node, we ask for its parent's evaluated value and add it to the evaluation of the single last attribute, which makes computations faster. Our request for the parent's value is never denied because the structure of the prefix tree makes sure its parent must have been evaluated. The detailed algorithm is shown in Algorithm \ref{alg:dictionary_calculations}.

\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    // Step1: This is pre-computing. Once per ML \\
    \Input{The root of the prefix tree during the compression stage of LZW}
	tree-node-list = [root] \\
	dic-entry-array = []    \\
	idx = 0                 \\
	\While {tree-node-list not empty} {
		node = tree-node-list.pop\_front() \\
		\If {node has been outputed as a code} {
			dict-entry-array[idx] = node \\
			idx += 1
		}
		\For {child of node} {
			child.set\_prefix\_idx(idx) \\
			tree-node-list.push\_back(child)
		}
	}
    // Step2: This is invoked basically once per iteration \\
    calculated-values=[] \\
    \For {i = 0 to len(dic-entry-array)} {
        \eIf {dic-entry-array[i] has prefix\_idx} {
            calculated-values[i] = calculated-values[prefix\_idx] + func(last attr value of dic-entry-array[i])
        } {
            calculated-values[i] = func(last attr value of dic-entry-array[i])
        }
    }
    \caption{Efficiently Precompute Intermediate Results on Dictionary Entries}
    \label{alg:dictionary_calculations}
\end{algorithm}


\noindent \textbf{Complexity of Our Solution}
By plugging $dist$/$weighted\_sums$ in $func$ in Algorithm \ref{alg:dictionary_calculations}, it is easy to compute the complexity of our solution as $O(|D|*k)$ and $O(|D|)$ respectively, where $|D|$ is the dictionary and k is the number of centroids. The naive way to evaluate $dist$/$weighted\_sums$ separately for each dictionary entry has complexity $O(|D|*k*\text{avg. len of dict entries})$ and $O(|D| * \text{avg. len of dict entries})$. Thus, theoretically speaking, our solution achieves a factor of the average length of dictionary entries speedup.

It's also important to note that our solution is cache friendly. In the second step of Algorithm \ref{alg:dictionary_calculations}, the access to calculated-values is consecutive because adjacent families of children are spawned by adjacent parents in the tree.

\noindent \textbf{Efficient Updating}. We introduce an efficient method to update the dictionary entries into the centroids/weight for Lloyd/GLMs. These updates happen at lines 14-16 in Algorithm~\ref{alg:kmeans-decoding} and lines 11-12 in Algorithm~\ref{alg:Compress_LogisticRegression}.


We discover similar structures as in efficient precomputing. That is, the updating operation using a dictionary entry X is ``decomposable'' and can be done by updating using the last attribute of X, and then postponing and aggregating the remaining attributes as a whole to the parent of X in the prefix tree.

Thus, we update machine learning models using the dictionary entries layer by layer from bottom to top in the prefix tree. For each entry, we only update using the last attribute and postpone/aggregate the remaining part of attributes to its parent. In this process, we only need to update each entry once because the structure of the prefix tree makes sure all the parents of the entry must have been updated beforehand. Algorithm \ref{alg:efficient_updating} shows the details of our solution.


\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    // Step1: We reuse the dic-entry-array in Algorithm \ref{alg:dictionary_calculations}. \\
    // Step2: This is invoked basically once per iteration \\
    update-scalar-vec // this should be pre-poluated by ML models \\
    \For {i = dic-entry-array.end to head} {
        \If {dic-entry-array[i] has prefix\_idx} {
            update-scalar-vec[prefix\_idx] += update-scalar-vec[i]
        }
        \textbf{update}(last attr value of dic-entry-array[i], update-scalar-vec[i])
    }
    \caption{Efficiently Update Machine Learning Models Using Dictionary Entries}
    \label{alg:efficient_updating}
\end{algorithm}

By plugging updating functions for Lloyd/GLM in \textbf{update} in Algorithm \ref{alg:efficient_updating}, the complexity of our updating algorithm is $O(|D|*k)$ and $(|D|)$ for Lloyd/GLM respectively, where $|D|$ is the dictionary and k is the number of centroids. On the other hand, the naive way to update the ML models using each dictionary entry separately has complexity $O(|D|*k*\text{avg. len of dict entries})$ and $O(|D|*\text{avg. len of dict entries})$ for Lloyd and GLM. Thus, again, our method could be the average length of dictionary entries times faster in theory.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% tombstone %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\eat{
A key insight that we observe is if X exists in the dictionary, then all its prefixes/dependencies must also exist in the dictionary. This is formally stated as the following theorem.
\begin{theorem}
Suppose there is a dictionary entry 

$X=[start\_idx, x_0, x_1, ..., x_n]$, then all the prefixes of $X$, 

$[start\_idx, x_0]$, $[start\_idx, x_0, x_1]$, ..., 

$[start\_idx, x_0, x_1, ..., x_{n-1}]$ must also exist in the dictionary.
\end{theorem}
\begin{proof}
We assume that the statement is false, then there must be a longest prefix $P$ of $X$ that doesn't exist in the dictionary. Denote $P$ as $[start\_idx, x_0, x_1, ..., x_p]$, then $[start\_idx, x_0, x_1, ..., x_p, x_{p+1}]$ must exist in the dictionary. In Algorithm \ref{alg:encoding}, when $[start\_idx, x_0, x_1, ..., x_p, x_{p+1}]$ is added to the prefix tree, $P$ must already exist in the prefix tree and is going to be outputed. Thus $P$ is a dictionary. This contradicts with the assumption that $P$ is not in the dictionary. Thus all the prefixes of $X$ must be in the dictionary.
\end{proof}
Since all the prefixes/dependencies of all the dictionary entries are also dictionary entries, we can solve this dynamic programming problem by evaluating the dictionary entries in the topological order of the dependency graph of the dictionary entries (for example, $[start\_idx, x_0, x_1, ..., x_n]$ depends on $[start\_idx, x_0, x_1, ..., x_{n-1}]$).
}

\eat{
We can easily verify this by examing $dist/weighted\_sums$ functions explicitly.
\begin{equation}
\begin{split}
    dist(X) =
    \begin{bmatrix}
        l_2(X.values, C_{|X.values}^0)^2 & \\
        l_2(X.values, C_{|X.values}^1)^2 & \\
        \vdots                            \\
        l_2(X.values, C_{|X.values}^k)^2 &
    \end{bmatrix}
\end{split}
\end{equation}

and

\begin{equation}
    weighted\_sums(X) = W_{|X.values}' X.values
\end{equation}
, where $C_{|X.values}^i$ denotes the corresponding values in ith centroids for X.values and $W_{|X.values}$ denotes the corresponding weights for X.values. 
}











==> toc.tex <==
We now introduce our tuple-oriented coding (TOC) scheme. We first introduce two key differences with the original LZW algorithm, then we explain our coding scheme in detail. Finally we give an example of running our coding scheme on a toy dataset.

\subsection{Two Departures from LZW} \label{sec:naive_encoding}

The first difference is that TOC respects tuple boundaries. Drawing inspiration from LZW, we treat the given training dataset \textbf{T} as a data file with the data serialized in row-major (tuple-oriented) order. However, as a key departure from LZW and text compression, we also track and maintain tuple boundaries in \textbf{T}, which are needed for ML. Thus, we introduce a new coding scheme we call tuple-oriented coding (TOC). Using a shared \textit{dictionary}, we encode the data file but prevent the encoding from crossing tuple boundaries.

The second difference is that dictionary entries in TOC are more complicated. Each entry in the dictionary has a \textit{code number} and a $2$-tuple: $(startIndex, values)$, wherein $values$ is a sequence of feature values that occurs contiguously in some tuple of \textbf{T} and $startIndex$ is the column index of the first feature in $values$. $startIndex$ is needed to align $values$ with ML model parameters. For example, if the sequence $[c,d]$ of the tuple $[a,b,c,d,e]$ is chosen to be represented as a code, the 2-tuple for it in the dictionary will be $(2, [c,d])$. The code numbers start from $0$ and identify each entry uniquely.

\subsection{TOC Encoding}
TOC starts by initializing with one entry for each unique feature value in \textbf{T}, i.e., sequences of length one each. The encoding algorithm adds new entries to the dictionary on the fly such that each new sequence is obtained by suffixing one feature value to some pre-existing entry's sequence. For example, $(2, [c,d])$ is added only if $(2, [c])$ is already present in the dictionary. Apart from being able to access the entry for a given code number, the dictionary also exposes the following two functions:
%
\begin{packeditems}
\item $C'$ = \textbf{AddDict}(C, v). Create a new dictionary entry by extending the sequence of an existing entry with code number C with v and return the new code number. 
If C is -1, the added entry's sequence is just v.

\item $C'$ = \textbf{GetIndex}(C, v). Return the code number of the sequence obtained by extending the sequence of an existing entry with code number C with v. 
If no such extended entry exists, return -1.

%\item W = \textbf{GetSequence}(C) Returns the sequence of values corresponding to index C.
\end{packeditems}
%
% \vspace{1mm}
The encoding scheme is presented in Algorithm~\ref{alg:encoding}. The first step initializes the dictionary with an entry for each starting index (lines 2-3) and then each entry for each unique feature value in \textbf{T} (lines 4-7). 
In the second step, for each tuple, for each feature yet to be encoded, we find the longest match $W$ in the dictionary using the subroutine \textbf{GetLongestMatch} shown in Algorithm~\ref{alg:long}. 
Once we hit a feature $t[i]$ ($i$ is returned in line 12) that cannot be matched, we add a new entry to the dictionary with the sequence $[W, t[i]]$. We then output the code number corresponding to $W$ to represent the compressed portion of the tuple. This process continues till the whole tuple is encoded. We denote the encoded table \textbf{T} as \textbf{T'}.

\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \Input{Denormalized table \textbf{T}, Number of features d}
    //Step 1: Initialize dictionary \\
    \For {i = 0; i $<$ d; i++} {
        \textbf{AddDict}(-1, i) \hfill // Add starting indexes \\
    }
    \For {tuple t in \textbf{T}} {
        \For{i = 0; i $<$ d; i++} {
            \If{\textbf{GetIndex}(i, t[i]) = -1} {
                \textbf{AddDict}(i, t[i]) \hfill // Unique feature values
            }
        }
    }
    //Step 2: Compress \textbf{T} \\
    \For {tuple t in \textbf{T}} {
        i =  0 \\
        \While{i $<$ d} {
            (C, i) = \textbf{GetLongestMatch}(i, t, d) \\
            \If{i $<$ d} {
                \textbf{AddDict}(C, t[i])
            } 
            \textbf{Output}(C)
        }
    }
    \caption{TOC Encoding}
    \label{alg:encoding}
\end{algorithm}

\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \Input{Starting index i, Tuple t, d}
    C' = \textbf{GetIndex}(i, t[i]) \\
    \While {C' $\neq$ -1} {
        (C, i) = (C', i + 1) \\
        \eIf {i $<$ d} {
            C'= \textbf{GetIndex}(C, t[i])
        } {
        C' = -1
    }
}
\Return{(C, i)}
\caption{\textbf{GetLongestMatch}}
\label{alg:long}
\end{algorithm}

\vspace{1mm}
\noindent \textbf{Example.} Figure~\ref{fig:encoding_example} gives a step-by-step example of how TOC encoding works on a toy dataset with two tuples.

\begin{figure}[th!]
\centering
    \includegraphics[width=0.6\linewidth]{./plots/cexample.pdf}
\vspace{2mm}
    \caption{Illustration of TOC encoding. \textbf{T} has two tuples: $[a, b, c, d, e]$ and $[f, g, c, d, e]$. \textbf{GetLM} is the output of \textbf{GetLongestMatch} for the symbol t[i]. \textbf{AddDict} shows the entry - $code\_number (start\_idx, [attrs])$ added to the dictionary upon finding a longest match, where $start\_idx$ is the column index of the first attribute. We omit Step 1, which initializes the dictionary with starting indexes: $0 (-1, 0)$, $1 (-1, 1)$, $2 (-1, 2)$, $3 (-1, 3)$, and $4 (-1, 4)$, as well as single-symbol sequences: $5 (0, [a])$, $6 (1, [b])$, $7 (2, [c])$, $8 (3, [d])$, $9 (4, [e])$, $10 (0, [f])$, and $11 (1, [g])$. Subsequent steps add more entries that extend these sequences. As an example, the first row shows that the longest match for $a$ is code number $5$, which resulted in the addition of a new entry $(0, [a, b])$ with code number $12$. The highlighted row in Step 1 and 2 is where we keep the boundaries of the tuple. That is, when the boundary of a tuple is reached, we stopped matching more characters in \textbf{GetLongestMatch} or adding a new entry in \textbf{AddDict}. Overall, the compressed tuples are $[5, 6, 7, 8, 9]$ and $[10, 11, 14, 9]$}
\label{fig:encoding_example}
\vspace{-3mm}
\end{figure}


